Virtual Linking Bids for Market Clearing with Non-Merchant Storage

In the context of energy market clearing, non-merchant assets are assets that do not submit bids but whose operational constraints are included. Integrating energy storage systems as non-merchant assets can maximize social welfare. However, the disconnection between consecutive market clearings poses challenges for market properties, and this is not well studied yet. We contribute to the literature on market clearing with non-merchant storage by proposing a market-clearing procedure that preserves desirable market properties, even under uncertainty. This approach is based on a novel representation of storage systems in which the energy available is discretized to reflect the different prices at which the storage system was charged. These prices are then included as virtual bids, establishing a link between different market clearings. We show that market clearing with such virtual linking bids has the advantage of guaranteeing cost recovery for market participants and can outperform traditional approaches in terms of social welfare.

==> sections/simult_proof.tex <==
\subsection{Simultaneous Charge and Discharge} \label{sec:scd}

% Meaning of simultaneous charge and discharge
Note that in the model in \eqref{prob:mc_vos}, $p_t\up{C,a}$ and $p_{vt}\up{D,e}$ can be positive at the same time, which corresponds to simultaneous charge and discharge of the inter- and intra-storages. However, this separation of the storage system is only a modeling artifice and has no physical meaning. It is the sum of the two that corresponds to the instruction of charge or discharge for the storage system. 

% Impact of negative values
Allowing the intra-storage system to take negative values generates multiple optimal solutions for which the sum of intra- and inter-storage is the same. It is possible to select among all these solutions one for which there is no simultaneous charge and discharge, by minimizing the total quantity exchanged or by introducing binary variables to choose between charge and discharge. We formalize this result with a proposition.

\begin{proposition} \label{proposition}
    For the market clearing in \eqref{prob:mc_vos}, and under the assumptions that the value of stored energy is strictly positive, i.e., $S_v > 0$, $\forall v \in \mathcal{V}$, and that a feasible solution exists, there will always be an optimal solution where the intra-storage does not charge when the inter-storage discharges.
\end{proposition}

\begin{proof}
    See Appendix.
\end{proof}

% Remark for S_v<=0
Note that $S_v=0$ is equivalent to not valuing the stored energy, in which case we can equivalently use the original formulation in which there is no separation between intra- and inter-storage and thus no simultaneous charge and discharge of intra- and inter-storage.
$S_v<0$ could also be treated in the same way as $S_v=0$ since it is unlikely that it is optimal for the storage system to discharge at a negative price and that it gets paid with a lower price than this $S_v<0$. 
